Splitting Steepest Descent for Growing Neural Architectures

We develop a progressive training approach for neural networks which adaptively grows the network structure by splitting existing neurons to multiple off-springs. By leveraging a functional steepest descent idea, we derive a simple criterion for deciding the best subset of neurons to split and a splitting gradient for optimally updating the off-springs. Theoretically, our splitting strategy is a second-order functional steepest descent for escaping saddle points in an $\infty$-Wasserstein metric space, on which the standard parametric gradient descent is a first-order steepest descent. Our method provides a new computationally efficient approach for optimizing neural network structures, especially for learning lightweight neural architectures in resource-constrained settings.

==> tex/experiment.tex <==
\section{Experiment}
\subsection{1D Toy}
We firstly generate 2000 synthesis data $(x_i, y_i)$ using 15 random $w_j = (w_{j1}, w_{j2})$. 
$$y_i = \sum_{j=1}^{15}K(w_{j}, x)$$
Where $$K(w_j, x) = e^{-||w_{j1}x - w_{j2}||^2}$$
Then, we pre-train a model using 10 random initialized $w^'$, that is using 

$$y_i' = \sum_{p=1}^{10}K(w'_p, x_i)$$
to train and estimate the data using gradient descent.

After the loss becomes stable, we calculate each $w$ 's eigen value, each time split one of them, and check the loss decrease after splitting and training. The following figure shows the relationship between the neuron's eigenvalue and the percent of loss decrease.
\textbf{[TODO: refine figure 1(b), add average result to Figure 2]}
\begin{figure*}[htb]
\centering
\begin{subfigure}{0.3\textwidth}
\includegraphics[width =\textwidth]{figure/eigen_performance.png}\caption{}\label{fig:pr_1d}
\end{subfigure}
\begin{subfigure}{0.3\textwidth}
\includegraphics[width = \textwidth]{figure/direction.png}\caption{}\label{fig:prgb_1d}
\end{subfigure}
\begin{subfigure}{0.3\textwidth}
\includegraphics[width = \textwidth]{figure/loss_curve.png}\caption{}\label{fig:loss_1d}
\end{subfigure}
\caption{(a) eigen value vs performance improvement, (b) direction of the smallest eigen value vs loss decrease, (c) loss curve}
\label{fig:random_exp}
\end{figure*}

We can see from the figure, the minimum eigen value has the greatest improvement after the split while the eigenvalue that near zero or positive do not have any improvement.


Moreover, we also check the loss decrease value vs split direction. In \ref{fig:toy_direction}, we can see that when the angle is 0, 180 and 360 degrees, which means the eigen vector direction, it can reach the biggest loss decrease. 

We additionally do a experiment that start from three $w'_j$, split one of them when the gradients less than a threshold. Comparing the loss curve of the random split and ours. 
Combine with the eigenvalue vs performance curve, we can see that if the split point is the position that has a big minimum eigenvalue, the split can hardly improve the effect, that is why the random split can not perform as good as us when split for a lot of time.


In addition, we want to exam whether we can use softplus function to approximate $ReLU$ activation when calculating $A$. We firstly sythseis some data using
$$y_i = \sum_{j=1}^{15}v_{j}\sigma(w_{j}x +b_j)$$
Where 
$$\sigma(x) = ReLU(x)$$
Then, we initial 6 neurons to fit the data. This time, we split $w_{j}$ by calculating the eigen value of $w_{j}$. When calculating $A$, we use $$\sigma '(x) = \frac{1}{a}ln(1 + e^{ax})$$ to approximate $\sigma(x)$,  the eigen value and loss changes is showed as following. 

\subsection{2D Toy model}
We try 2D MMD on fitting Gaussian Mixture model. We start from one single particle, split it when its gradient is near zero. We compare this method with random splitting and jointly train all of the particles. We setup a 3-components GMM, to clearly see the different, we set three components differ from each other, that means one of the components is very wide while another one is very sharp. In splitting methods, the particle will become smaller which shows that its weight become small after splitting. 

\begin{figure*}[htb]
\centering
\begin{subfigure}{0.3\textwidth}
\includegraphics[width =\textwidth]{figure/joint.png}\caption{jointly}\label{fig:joint_2d}
\end{subfigure}
\begin{subfigure}{0.3\textwidth}
\includegraphics[width = \textwidth]{figure/randomsp.png}\caption{random split}\label{fig:randomsp_2d}
\end{subfigure}
\begin{subfigure}{0.3\textwidth}
\includegraphics[width = \textwidth]{figure/oursp.png}\caption{ours}\label{fig:oursp_2d}
\end{subfigure}
\caption{Different method to fit the MMD}
\label{fig:random_exp}
\end{figure*}


\begin{figure*}[htb]
\centering
\begin{subfigure}{0.3\textwidth}
\includegraphics[width =\textwidth]{figure/pad_30.png}\caption{random initialization}\label{fig:joint_2d}
\end{subfigure}
\begin{subfigure}{0.3\textwidth}
\includegraphics[width = \textwidth]{figure/random_30.png}\caption{random split}\label{fig:randomsp_2d}
\end{subfigure}
\begin{subfigure}{0.3\textwidth}
\includegraphics[width = \textwidth]{figure/our_30.png}\caption{ours}\label{fig:oursp_2d}
\end{subfigure}
\caption{Different method to fit the MMD}
\label{fig:random_exp}
\end{figure*}
\textbf{[TODO:loss curv]}
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
\hline  
Method&jointly&random split& random initialization & ours \\
\hline  
Loss& 0.05421 & 0.06643 & 0.06032 & \textbf{0.04424}\\
\hline 
\end{tabular}
\end{center}

\subsection{Fashion-MNIST}
We then set a 2 hidden layer fully connected nerual networks on Fasion MNIST dataset. We begin at a very small network, observing the performance under different split setting.


==> tex/intro.tex <==
\section{Introduction}
\label{sec:intro}
